NELA-GT-2020: A Large Multi-Labelled News Dataset for The Study of Misinformation in News Articles

In this paper, we present an updated version of the NELA-GT-2019 dataset, entitled NELA-GT-2020. NELA-GT-2020 contains nearly 1.8M news articles from 519 sources collected between January 1st, 2020 and December 31st, 2020. Just as with NELA-GT-2018 and NELA-GT-2019, these sources come from a wide range of mainstream news sources and alternative news sources. Included in the dataset are source-level ground truth labels from Media Bias/Fact Check (MBFC) covering multiple dimensions of veracity. Additionally, new in the 2020 dataset are the Tweets embedded in the collected news articles, adding an extra layer of information to the data. The NELA-GT-2020 dataset can be found at https://doi.org/10.7910/DVN/CHMUYZ.

==> tex/labels_legend_table.tex <==
\newgeometry{left=2cm, top=1.4cm}

\begin{table*}[!ht]
    \fontsize{9}{9.2}\selectfont  % fontsize, spacing
    \renewcommand{\arraystretch}{1.4}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[t]{L{3.6cm}lL{10.4cm}C{2.5cm}}
        \textbf{Section} & & \textbf{Description} \hfill (NewsGuard points) & \textbf{Coloring} \\ \hline
        %
        NewsGuard 
        & ~~1. & Does not repeatedly publish false content \hfill (22.0)  & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~2. & Gathers and presents information responsibly \hfill (18.0) &  \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~3. & Regularly corrects or clarifies errors \hfill (12.5)  &                                 \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~4. & Handles the difference between news and opinion responsibly \hfill (12.5)  &            \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~5. & Avoids deceptive headlines \hfill (10.0) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~6. & Website discloses ownership and financing \hfill (7.5) &                               \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~7. & Clearly labels advertising \hfill (7.5) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~8. & Reveals who's in charge, including any possible conflicts of interest \hfill (5.0) &   \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~9. & Provides information about content creators \hfill (5.0) &                             \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& 10. & Aggregated \texttt{score} computed from 1-9 & \includegraphics[width=1.6ex]{fig/colors/green.pdf} - \includegraphics[width=1.6ex]{fig/colors/purple.pdf} ~~ \\
    	& 11. & Column 10 thresholded at 60 points &
    	\includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
    	% 
    	Pew Research Center 
    	& 12. & Trust from consistently-liberals & \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 13. & Trust from mostly-liberals & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 14. & Trust from mixed groups & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 15. & Trust from mostly-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 16. & Trust from consistently-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 17. & Aggregated trust from 12-16 & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Wikipedia 
        & 18. & Existence of source on Wikipedia's list of fake news sources & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Open Sources 
        & 19. & Marked reliable & \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\
        & 20. & Marked blog & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 21. & Marked clickbait & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 22. & Marked rumor & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 23. & Marked fake & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 24. & Marked unreliable & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 25. & Marked biased & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 26. & Marked conspiracy & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 27. & Marked hate speech & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 28. & Marked junk science & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 29. & Marked political & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 30. & Marked satire & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 31. & Marked state news & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\ \hline
        %
        Media Bias / Fact Check 
        & 32. & Factual reporting from 5 (good) down to 1 (bad) & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 33. & Special label; conspiracy, pseudoscience or questionable source (purple), and satire (orange) &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 34. & Political leaning / bias from left to right. & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        Allsides 
        & 35. & Political leaning / bias & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        BuzzFeed
        & 36. & Political leaning / bias, but only left and right &
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        PolitiFact
        & 37. & Has brought story labelled as "pants on Fire!" &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 38. & Has brought story labelled as false &
        \includegraphics[width=1.6ex]{fig/colors/purple2_grey.pdf} \\
        & 39. & Has brought story labelled as mostly false &
        \includegraphics[width=1.6ex]{fig/colors/purple_grey2.pdf} \\
        & 40. & Has brought story labelled as half-true &
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 41. & Has brought story labelled as mostly true &
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} \\
        & 42. & Has brought story labelled as true &
        \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\ \hline
        %
        Alexa Ranking & & The Alexa ranking of the source. & Numerical \\ \hline
        %
        \# Articles & & The number of articles collected from the source. & Numerical \\ \hline
        %
        First Observed & & The date of first articles collected from the source. & dd-mm-yyyy \\ \hline
    \end{tabular}
    \caption{Details of the information for sources found in tables \ref{tab:source_labels1}, \ref{tab:source_labels2} and \ref{tab:source_no_labels}. We generally use green-to-purple for good-to-poor reliability/credibility, with grey as inconclusive. For bias we use blue-to-red for left-to-right bias, with grey as unbiased. Orange is used for special cases. In NewsGuard data it represents missing information, in Open Sources it marks auxiliary labels and for Media Bias / Fact Check it marks satire. }
    \label{tab:labelling_explanations}
\end{table*}

\restoregeometry

